Toward Semi-Automatic Misconception Discovery Using Code Embeddings

Understanding students' misconceptions is important for effective teaching and assessment. However, discovering such misconceptions manually can be time-consuming and laborious. Automated misconception discovery can address these challenges by highlighting patterns in student data, which domain experts can then inspect to identify misconceptions. In this work, we present a novel method for the semi-automated discovery of problem-specific misconceptions from students' program code in computing courses, using a state-of-the-art code classification model. We trained the model on a block-based programming dataset and used the learned embedding to cluster incorrect student submissions. We found these clusters correspond to specific misconceptions about the problem and would not have been easily discovered with existing approaches. We also discuss potential applications of our approach and how these misconceptions inform domain-specific insights into students' learning processes.

==> table/generalGrading.tex <==
\begin{table}
\centering
\caption{General grading accuracy (A), precision (P), recall (R), area under ROC curve (AUC), F-1 Score (F1) for code2vec and attention network.}
\label{table:grading_all}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
                   & \textbf{Major} & \textbf{SVM} & \textbf{NN} & \textbf{C2V} &  \textbf{Att}        \\ \hline
\textbf{A}  & 63.95\%    & 69.67\% & 71.71\%       & 75.66\%                 & \textbf{75.80\%}                    \\ \hline
\textbf{P}  & 0  & 61.68\% & 62.74\%         & \textbf{67.06\%}   & 62.35\%    \\ \hline
\textbf{R} & 0  & 42.21\% & 58.30\% & 72.66\%            & \textbf{77.55\%}   \\ \hline
\textbf{AUC} & 0.5 & 0.650 & 0.689 & 0.814 & \textbf{0.838} \\ \hline
\textbf{F1} & 0  & 0.460 & 0.593 & \textbf{0.6895} & 0.686 \\ \hline
\end{tabular}
\end{table}


==> table/gradingAccuracy.tex <==

\begin{table}
\centering
\caption{Grading accuracy for rubric items in code2vec and attention network.}
\label{table:grading_acc_rubric}
\begin{tabular}{|c|c|c|c|}
\hline
                   &\textbf{Majority}  & \textbf{Code2vec} & \textbf{Attention}  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}1 Block\\  Input\end{tabular}} & 75.48\% &  87.62\% & \textbf{\begin{tabular}[c]{@{}c@{}}90.71\%\\  (+3.09\%)\end{tabular}} \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Pen\\ Down\end{tabular}} & 80.48\% & 79.28\% & \textbf{\begin{tabular}[c]{@{}c@{}}86.30\%\\  (+7.02\%)\end{tabular}} \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Variable\\ Init\end{tabular}} & 88.33\%  & 90.47\% & \textbf{\begin{tabular}[c]{@{}c@{}}94.76\%\\  (+4.29\%)\end{tabular}} \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}Repeat \\ Rotations\end{tabular}} & 47.86\%  & 80.95\% & \textbf{\begin{tabular}[c]{@{}c@{}}81.42\%\\  (+0.47\%)\end{tabular}}\\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}Move \\ + Turn\end{tabular}} & 84.29\% & \textbf{87.38\%} & \begin{tabular}[c]{@{}c@{}}83.92\% \\  (-3.46\%)\end{tabular}\\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}Variable \\ Increment\end{tabular}} & 82.38\% & 87.85\% & \textbf{\begin{tabular}[c]{@{}c@{}}90.95\%\\  (+3.10\%)\end{tabular}} \\ \hline
\end{tabular}
\end{table}

% \begin{table}
% \centering
% \caption{Grading accuracy for rubric items in code2vec and attention network.}
% \label{table:grading_acc_rubric}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
%                   &\textbf{Major} &\textbf{SVM} &\textbf{NN}  & \textbf{C2V} & \textbf{Att}  \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}1 Block\\  Input\end{tabular}} & 75.48\% & 83.09\% & 84.52\% &  87.62\% & \textbf{\begin{tabular}[c]{@{}c@{}}90.71\%\\  (+3.09\%)\end{tabular}} \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}Pen\\ Down\end{tabular}} & 80.48\% & 85.71\% & 80.00\% & 79.28\% & \textbf{\begin{tabular}[c]{@{}c@{}}86.30\%\\  (+7.02\%)\end{tabular}} \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}Variable\\ Init\end{tabular}} & 88.33\% & 92.02\% & 88.69\%  & 90.47\% & \textbf{\begin{tabular}[c]{@{}c@{}}94.76\%\\  (+4.29\%)\end{tabular}} \\ \hline

% \textbf{\begin{tabular}[c]{@{}c@{}}Repeat \\ Rotations\end{tabular}} & 47.86\% & 72.97\% & 72.26\%  & 80.95\% & \textbf{\begin{tabular}[c]{@{}c@{}}81.42\%\\  (+0.47\%)\end{tabular}}\\ \hline

% \textbf{\begin{tabular}[c]{@{}c@{}}Move \\ + Turn\end{tabular}} & 84.29\% & 83.57\% & 85.11\% & \textbf{87.38\%} & \begin{tabular}[c]{@{}c@{}}83.92\% \\  (-3.46\%)\end{tabular}\\ \hline

% \textbf{\begin{tabular}[c]{@{}c@{}}Variable \\ Increment\end{tabular}} & 82.38\% & 89.76\% & 85.83\% & 87.85\% & \textbf{\begin{tabular}[c]{@{}c@{}}90.95\%\\  (+3.10\%)\end{tabular}} \\ \hline
% \end{tabular}
% \end{table}

==> table/gradingAccuracyLAK.tex <==

\begin{table}
\centering
\caption{Grading accuracy for rubric items in code2vec.}
\label{table:grading_acc_rubric_lak}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Rubric Item}                    &\textbf{Majority}  & \textbf{SVM}& \textbf{NN} & \textbf{Code2vec}   \\ \hline
\textbf{1 Block Input}                  & 75.48\%           &  81.54\%    &  85.23\%    & \textbf{87.62\%}  \\ \hline
\textbf{Variable Init}                  & 80.48\%           &  \textbf{87.02\%}    &  76.90\%    & 79.28\% \\ \hline
\textbf{Move + Turn}                    & 88.33\%           &  \textbf{92.61\%}    &  89.28\%    & 90.47\%  \\ \hline

\textbf{Repeat Rotations}               & 47.86\%           &  75.35\%    &  73.09\%    & \textbf{80.95\%} \\ \hline

\textbf{Pen Down}                       & 84.29\%           &  83.33\%    &  84.40\%    & \textbf{87.38\%} \\ \hline

\textbf{Variable Increment}             & 82.38\%           &  \textbf{88.92\%}    &  85.23\%    & 87.85\%  \\ \hline
\end{tabular}
\end{table}

==> table/gradingAll.tex <==

\begin{table}
\centering
\caption{Metrics of general grades in transfer learning.}
\label{table:transfer_all}
\begin{tabularx}{.2\textwidth}{|c|c|}

\hline
                   & \textbf{Metrics}         \\ \hline
\textbf{Accuracy}  & 75.57\%                      \\ \hline
\textbf{Precision}  & 62.97\%       \\ \hline
\textbf{Recall} & 75.37\%    \\ \hline
\textbf{AUC} & 0.8240  \\ \hline
\textbf{F1} & 0.6771 \\ \hline
\end{tabularx}
\end{table}

==> table/precisionRecall.tex <==

\begin{table}
\label{table:precisionRecall}

\centering
\caption{Precision(P), recall(R), and the top-$2$ frequent operations for rubric items in expert and model labels.}
\label{table:feedback_rubric}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|}
\hline
                                                                           \textbf{Rubric}                 & \multicolumn{2}{c|}{\textbf{Metric}} & \textbf{Expert}      & \textbf{Machine}  \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}1 Block\\ Input\end{tabular}}}           & \textbf{P} & 0.32          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{customBlock}\\ \texttt{varDec}\end{tabular}}     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{customBlock}\\ \texttt{doRepeat}\end{tabular}} \\ \cline{2-3}
                                                                                            & \textbf{R}    & 0.88          &                                                                                   &                                                                                      \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Pen\\ Down\end{tabular}}}                & \textbf{P} & 0                & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{customBlock}\\ \texttt{down}\end{tabular}}       & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{doSetVar}\\ \texttt{doChangeVar}\end{tabular}}               \\ \cline{2-3}
                                                                                            & \textbf{R}    & 0                &                                                                                   &                                                                                      \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Variable\\ Init\end{tabular}}} & \textbf{P} & 0.37          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{doSetVar}\\ \texttt{customBlock}\end{tabular}}   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{doSetVar}\\ \texttt{customBlock}\end{tabular}}          \\ \cline{2-3}
                                                                                            & \textbf{R}    & 0.50          &                                                                                   &                                                                                      \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Repeat\\ Rotations\end{tabular}}}  & \textbf{P} & 0.97            & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{doRepeat}\\ \texttt{reportProduct}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{doRepeat}\\ \texttt{reportProduct}\end{tabular}}    \\ \cline{2-3}
                                                                                            & \textbf{R}    & 0.98          &                                                                                   &                                                                                      \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Move\\ + Turn\end{tabular}}}             & \textbf{P} & 0.58          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{doRepeat}\\ \texttt{forward}\end{tabular}}       & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{doRepeat}\\ \texttt{reportProduct}\end{tabular}}    \\ \cline{2-3}
                                                                                            & \textbf{R}    & 0.25          &                                                                                   &                                                                                      \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Variable\\ Increment\end{tabular}}}      & \textbf{P} & 0.64          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{doChangeVar}\\ \texttt{doRepeat}\end{tabular}}   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{doChangeVar}\\ \texttt{doSetVar}\end{tabular}}   \\ \cline{2-3}
                                                                                            & \textbf{R}    & 0.71          &                                                                                   &                                                                                      \\ \hline
\end{tabular}
\end{table}


==> table/snapDistribution.tex <==
\begin{table}
\centering
\caption{Grade distribution of rubric items.}
\label{table:snapdistribution}
\begin{tabular}{|c|c|c|c|}
\hline
        &\textbf{\begin{tabular}[c]{@{}c@{}}1 Block \\ Input\end{tabular}}&
        \textbf{\begin{tabular}[c]{@{}c@{}}Pen\\ Down\end{tabular}}&
        \textbf{\begin{tabular}[c]{@{}c@{}}Variable\\ Init\end{tabular}} \\ \hline
        \textbf{Correct rate}&
        \begin{tabular}[c]{@{}c@{}}158\\ (76.32\%)\end{tabular}&
        \begin{tabular}[c]{@{}c@{}}165\\ (79.71\%)\end{tabular}&
        \begin{tabular}[c]{@{}c@{}}186\\ (89.86\%)\end{tabular} \\ \hline

        &\textbf{\begin{tabular}[c]{@{}c@{}}Repeat\\ Rotations\end{tabular}}&
        \textbf{\begin{tabular}[c]{@{}c@{}}Move +\\ Turn\end{tabular}}&
        \textbf{\begin{tabular}[c]{@{}c@{}}Variable\\ Increment\end{tabular}} \\ \hline
        \textbf{\begin{tabular}[c]{@{}c@{}}Correct count \\ (rate)\end{tabular}}&
        \begin{tabular}[c]{@{}c@{}}100\\ (48.30\%)\end{tabular}&
        \begin{tabular}[c]{@{}c@{}}174\\ (84.06\%)\end{tabular}&
        \begin{tabular}[c]{@{}c@{}}167\\ (80.68\%)\end{tabular} \\ \hline
          
\end{tabular}
\end{table}

==> table/transferRubricAcc.tex <==
\begin{table}
\centering
\caption{Grading accuracy for rubric items for pre-trained LANN (and improvement over standard LANN).}
\label{table:transfer_rubric_acc}
\begin{tabular}{|c|c|c|c|}
\hline
        &\textbf{\begin{tabular}[c]{@{}c@{}}1 Block \\ Input\end{tabular}}&
        \textbf{\begin{tabular}[c]{@{}c@{}}Pen\\ Down\end{tabular}}&
        \textbf{\begin{tabular}[c]{@{}c@{}}Variable\\ Init\end{tabular} }\\ \hline
        \textbf{\begin{tabular}[c]{@{}c@{}}Accuracy \\ (Change) \end{tabular}}&
        \textbf{\begin{tabular}[c]{@{}c@{}}$92.02\%$ \\ (+1.31\%) \end{tabular}} &
        \textbf{\begin{tabular}[c]{@{}c@{}}$85.59\%$ \\ (-0.71\%) \end{tabular}} &
        \textbf{\begin{tabular}[c]{@{}c@{}}$94.16\%$ \\ (-0.60\%) \end{tabular}} \\ \hline

        &\textbf{\begin{tabular}[c]{@{}c@{}}Repeat\\ Rotations\end{tabular}}&
        \textbf{\begin{tabular}[c]{@{}c@{}}Move +\\ Turn\end{tabular}}&
        \textbf{\begin{tabular}[c]{@{}c@{}}Variable\\ Increment\end{tabular}} \\ \hline
        \textbf{\begin{tabular}[c]{@{}c@{}}Accuracy \\ (Change) \end{tabular}}&
        \textbf{\begin{tabular}[c]{@{}c@{}}$82.38\%$ \\ (+0.96\%) \end{tabular}} & 
        \textbf{\begin{tabular}[c]{@{}c@{}}$81.42\%$ \\ (-2.50\%) \end{tabular}} & 
        \textbf{\begin{tabular}[c]{@{}c@{}}$92.02\%$ \\ (+1.07\%) \end{tabular}} \\ \hline
          
\end{tabular}
\end{table}
